AssertionBench: A Benchmark to Evaluate Large-Language Models for Assertion Generation

Assertions have been the de facto collateral for simulation-based and formal verification of hardware designs for over a decade. The quality of hardware verification, \ie, detection and diagnosis of corner-case design bugs, is critically dependent on the quality of the assertions. There has been a considerable amount of research leveraging a blend of data-driven statistical analysis and static analysis to generate high-quality assertions from hardware design source code and design execution trace data. Despite such concerted effort, all prior research struggles to scale to industrial-scale large designs, generates too many low-quality assertions, often fails to capture subtle and non-trivial design functionality, and does not produce any easy-to-comprehend explanations of the generated assertions to understand assertions' suitability to different downstream validation tasks. Recently, with the advent of Large-Language Models (LLMs), there has been a widespread effort to leverage prompt engineering to generate assertions. However, there is little effort to quantitatively establish the effectiveness and suitability of various LLMs for assertion generation. In this paper, we present AssertionBench, a novel benchmark to evaluate LLMs' effectiveness for assertion generation quantitatively. AssertioBench contains 100 curated Verilog hardware designs from OpenCores and formally verified assertions for each design generated from GoldMine and HARM. We use AssertionBench to compare state-of-the-art LLMs to assess their effectiveness in inferring functionally correct assertions for hardware designs. Our experiments demonstrate how LLMs perform relative to each other, the benefits of using more in-context exemplars in generating a higher fraction of functionally correct assertions, and the significant room for improvement for LLM-based assertion generators.

==> code/prompt_old.tex <==
\begin{comment}
You are an expert in SystemVerilog Assertions.
Your task is to generate the list of assertions to the given verilog design. An example is shown below. Generate only the list of assertions for the test program with no additional text.
Program 1: module arb2(clk, rst, req1, req2, gnt1, gnt2); input clk, rst; input req1, req2; output gnt1, gnt2; reg state; reg gnt1, gnt2; always @ (posedge clk or posedge rst) if (rst) state <= 0; else state <= gnt1; always @ (*) if (state) begin gnt1 = req1 & ~req2; gnt2 = req2; end else begin gnt1 = req1; gnt2 = req2 & ~req1; end endmodule
Assertions 1: (state == 1 & req2 == 1) |-> (gnt1 == 0);(req1 == 1 & state == 0) |-> (gnt1 == 1);(req1 == 0) |-> (gnt1 == 0);(req1 == 1 & req2 == 0) |-> (gnt1 == 1);(req1 == 1 & state == 0) |-> (gnt2 == 0);(req2 == 1 & state == 1) |-> (gnt2 == 1);(req2 == 0) |-> (gnt2 == 0);(req2 == 1 & req1 == 0) |-> (gnt2 == 1); (gnt2) |-> (req2); (gnt1) |-> (req1); 
Test Program: 
module fifo_mem #(parameter DEPTH=8, DATA_WIDTH=8, PTR_WIDTH=3) ( input wclk, w_en, rclk, r_en, input [PTR_WIDTH:0] b_wptr, b_rptr, input [DATA_WIDTH-1:0] data_in, input full, empty, output 
reg [DATA_WIDTH-1:0] data_out); reg [DATA_WIDTH-1:0] fifo[0:DEPTH-1]; always@(posedge wclk) begin if(w_en & !full) begin fifo[b_wptr[PTR_WIDTH-1:0]] <= data_in; end end always@(posedge rclk) begin  data_out <= fifo[b_rptr[PTR_WIDTH-1:0]]; end endmodule
Test Assertions:
\end{comment}

==> pic/accuracy_across_LLMs.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[scale=0.25]{pic/1-shot_accuracy.pdf}
        \caption{1-shot.\label{fig:1_shot_acc}}
    \end{subfigure}
    %\hspace{6mm}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[scale=0.25]{pic/5-shot_accuracy.pdf}
        \caption{5-shot.\label{fig:5_shot_acc}}
    \end{subfigure}   
    \caption{{\bf Comparison of accuracy of generated assertions in terms of passing, failing, (generating a counter example), and syntactically wrong assertions between different LLMs per $k$-shot learning where $k = 1$ and $k = 5$}. %Comparison of accuracy of generated assertions over all the considered models $\gptt$, $\gptf$  
    }
    \label{fig:accuracy_across_LLMs}
\end{figure}

% \begin{wrapfigure}{r}{2.5in}
%     \centering
%     \begin{subfigure}[b]{0.3\textwidth}
%         \includegraphics[scale=0.18]{pic/1-shot_accuracy.pdf}
%         \caption{1-shot.\label{fig:exp_circuit_sweeps}}
%     \end{subfigure}
%     %\hspace{6mm}
%     \hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%         \includegraphics[scale=0.18]{pic/5-shot_accuracy.pdf}
%         \caption{5-shot.\label{fig:reconvergent}}
%     \end{subfigure}   
%     \caption{Caption}
%     \label{fig:accuracy_across_LLMs}
% \end{wrapfigure}

==> pic/assertion_evaluation.tex <==
\renewcommand{\arraystretch}{1.2}
\renewcommand{\columnsep}{10pt}
%\begin{wrapfigure}{r}{2.5in}
\begin{figure}
    \centering
    \resizebox{0.72\linewidth}{!}{
    \begin{tabular}{|cc|c|c|c|}
         \hline
         \multicolumn{3}{|c|}{}& \multicolumn{2}{|c|}{\bf Pre-condition}\\
         \cline{4-5}
         \multicolumn{3}{|c|}{} & {\bf Covered} & {\bf Unreachable}\\
         \hline
         \hline
         & & \multirow{2}{*}{\rotatebox[origin=c]{90}{{\centering \bf True}}} &  \multirow{2}{*}{\bf Valid} & \multirow{4}{*}{\centering \bf Vacuous}\\
         \multicolumn{2}{|c|}{\bf Post-} & %\multirow{2}{*}{\rotatebox[origin=c]{90}{{\centering \bf Condition}}} 
         &  & \\
         \cline{3-4}
         \multicolumn{2}{|c|}{\bf Condition} & \multirow{2}{*}{\rotatebox[origin=c]{90}{{\centering \bf False}}} & \multirow{2}{*}{\bf CEX} & \\
         & & & & \\
         \hline
    \end{tabular}
    }
    \caption{{\bf Assertion status based on pre-condition and post-condition evaluation}. {\bf CEX}: Counter example.}
    \label{tab:assertion_eval}
%\end{wrapfigure}
\end{figure}

==> pic/code_assertion_background.tex <==
\renewcommand{\columnsep}{16pt}
%\begin{wrapfigure}[22]{r}{2.8in}
\begin{figure}
\lstinputlisting[language=Verilog, 
                 linewidth=2.8in, framexleftmargin=2pt,
                 framexrightmargin=2pt,
                 ]{code/arb2.v}
\caption{{\bf A Verilog code for a 2-port Arbiter}~\cite{pal2020tcad}.}
\label{fig:arbiter_code}
%\end{wrapfigure}
\end{figure}

==> pic/comparative_results.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[]{}
%     \caption{Caption}
%     \label{fig:comparative_results}
% \end{figure}

==> pic/design_details.tex <==
% \begin{wrapfigure}{r}{3.0in}
%     \includegraphics[scale=0.3]{pic/design_details.pdf}
%     \caption{Caption}
%     \label{fig:accuracy_across_LLMs}
% \end{wrapfigure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{pic/design_details.pdf}
    \vspace{-4mm}
    \caption{{\bf Detail of the designs in the test set in terms of the number of lines of code (excluding comments and blank lines)}.}
    \label{fig:design_deatails}
    \vspace{-5mm}
\end{figure}


==> src/background.tex <==
\subsection{Background %\page{1}\assign{Debjit}
}\label{sec:background}

%% Talk about what is Assertion -- what is it -- explain with an example -- may be the arbiter itself. Talk about SystemVerilog Assertions (SVA) and talk about the subset that we are aiming for (sequence subset). Give some background of formal methods and how it filters invalid assertions

\input{pic/code_assertion_background}

In this section, we provide a few %preliminary 
definitions necessary to understand assertion generation and $\pname$. For our discussion, we consider a Verilog RTL design ${\cal D}$. ${\cal D}$ is a parallel composition of a set of concurrent processes $P_i$ ({\tt always} and {\tt assign} blocks), and let $V$ be the set of design signals. Let ${\cal I} \subset V$ be the set of input signals, 
${\cal O} \subset V$ be the set of output signals, and ${\cal R} \subset V$ be the set of internal registers. In~\Cref{fig:arbiter_code}, we show a Verilog design $\mathcal{D}$ of a 2-port Arbiter, consisting of %it consists of 
two concurrent {\tt always} processes $P_1$ (line 6) and $P_2$ (line 11), and $V = \{clk, rst, req1, req2, gnt1, gnt2, gnt\_\}$, $\mathcal{I} = \{clk, rst, req1, req2\}$, $\mathcal{O} = \{gnt1, gnt2\}$, and $\mathcal{R} = \{gnt\_\}$.

We define an \bem{assertion} in a restricted manner as that of~\cite{athavale2014dac}. An assertion is a temporal formula in LTL~\cite{ltl} of the format $P = \mathcal{G}(A \rightarrow C)$ where the antecedent $A$ is of the form $A = A_0 \wedge \mathcal{X}(A_1) \wedge \mathcal{X}\mathcal{X}(A_2) \wedge \ldots \wedge \mathcal{X}^m(A^m)$ and consequent $C$ is of the form $C = \mathcal{X}^n(C^n)$, where $n \geq m$. Each $A_i$ ($C_i$) is a proposition and is a $(v, val)$ pair where $v \in V$ and $val \in \{0, 1\}$. $\mathcal{X}$ is called the next-cycle operator and $\mathcal{X}^n (n \geq 0)$ is equal to a delay of $n$ clock cycles $\underbrace{\mathcal{X}\mathcal{X}\ldots\mathcal{X}}_{n~\text{times}}$.  We say an assertion $P$ is True if $\mathcal{D} \models P$ (read as $\mathcal{D}$ models $P$), in other words the assertion holds True globally (indicated by $\mathcal{G}$ operator) on design $\mathcal{D}$. Otherwise, the assertion is False, \ie, $\mathcal{D} \not\models P$ and there exists a Boolean value assignment to design signals known as $cex$ (counter example) that shows a refutation of assertion $P$ on $\mathcal{D}$. The implication operator $\rightarrow$ in $P$ could be of two types, {\em overlapped} and {\em non-overlapped}. The {\em overlapped} implication operator denoted as $\rightarrow$ implies {\em if there is a match on the antecedent $A$, then the consequent $C$ is evaluated in the same clock cycle}. The {\em non-overlapped} implication operator denoted as $\Rightarrow$ implies {\em if there is a match on the antecedent $A$, then the consequent $C$ is evaluated in the next clock cycle}. Additionally, based on the evaluation condition of the pre-condition and the post-condition, an assertion can have different evaluations. In~\Cref{tab:assertion_eval}, we show the assertion evaluation status. Note $A \rightarrow C$ can be re-written as $\neg A \vee C$. Consequently, if pre-condtion $A$ is {\bf unreachable} (or False), then the assertion $P$ is vacuously True (\ie, $\neg False \vee C$). If pre-condition $A$ is True and post-condition $C$ is True as well, the assertion is reported to be Valid %for design 
(\ie, $\mathcal{D} \models P$), otherwise, if the post-condition $C$ is False, then a counter example $cex$ is generated. %({\bf CEX}) is found which shows evidence how the design $\mathcal{D}$ refutes assertion $P$ (\ie, $\mathcal{D} \not\models P$).

\input{pic/assertion_evaluation}

For the Arbiter design of~\Cref{fig:arbiter_code}, consider two assertions $P1: \mathcal{G}((req1 == 1 \wedge req2 == 0) \rightarrow (gnt1 == 1))$ and $P2: \mathcal{G}((req2 == 0 \wedge gnt\_ == 1) \wedge \mathcal{X}(req1 == 1) \rightarrow \mathcal{X}(gnt1 == 1))$. The assertion $P1$ will evaluate to True if $req1$ is {\tt 1'b1} and $req2$ is {\tt 1'b0} at the current clock cycle, then $gnt1$ is {\tt 1'b1} in the current clock cycle. Note that $P1$ contains the {\em overlapped} implication operator $\rightarrow$. The assertion $P2$ will evaluate to True if $req2$ is {\tt 1'b0} and $gnt\_$ is {\tt 1'b1} in the current cycle, $req1$ is {\tt 1'b1} in the next cycle, then $gnt1$ is {\tt 1'b1} in the cycle after (\ie, in the $2^{nd}$ cycle). Note that $P2$ can be re-written using the {\em non-overlapped} implication operator in the following way $P2: \mathcal{G}((req2 == 0 \wedge gnt\_ == 1) \wedge \mathcal{X}(req1 == 1) \Rightarrow (gnt1 == 1))$ where the $\Rightarrow$ subsumes the $\mathcal{X}$ operator in %of 
the consequent. When we try to discharge a proof for $P1$ and $P2$ using a formal property verification (FPV) engine, such as Cadence JasperGold~\cite{jaspergold}, we find $P1$ is a valid assertion, \ie, $\mathcal{D} \models P1$ whereas JasperGold finds a counterexample (CEX) for $P2$, \ie, $\mathcal{D} \not\models P2$. We will use the assertion evaluation criterion of~\Cref{tab:assertion_eval} to define our {\em goodness} metric while evaluating SOTA LLMs for assertion generation task.



==> src/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer %these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a %{\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? %\answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? %\answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for %your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only %keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} This is described in Section 7.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{} We do not anticipate any negative societal impacts of this work.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{} Our paper does not include theoretical results.
	\item Did you include complete proofs of all theoretical results?
    \answerNA{} Our paper does not include theoretical results.
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} All data and software for this project is uploaded both as supplementary material and at the url provided.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} All experimental details are provided in Section 5.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} Described in Section 5.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
   \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{} We do not use crowdsourcing.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{} We do not use crowdsourcing.
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
   \answerNA{} We do not use crowdsourcing.
\end{enumerate}

\end{enumerate}

%\clearpage


==> src/related_work.tex <==
\subsection{Related Work %\page{0.75}\assign{Debjit}
}\label{sec:rel_work}

%% Talk about Assertion Generation Techniques -- Classical and then LLM-related 

%% Then explain that there is a lack of assertion benchmarks for training and validation. Mostly its prompt engineering without verifying whether generated assertions are correct/valid. Even we can mention that most require an extensive prompt engineering and human ingenuity.

Automatic generation of assertions in software and hardware has been an active area of research since seventies. Assertion generation via static analysis of design source code has been studied in the context of deductive program verification~\cite{bensalem1996powerful, caplain75, misra1977jaydev}. Static analysis techniques have been used to learn and generate likely program invariants for software verification~\cite{tiwari2004tacas, spin2004}. Data Mining and data-driven dynamic analysis have also been used to generate software invariants. DAIKON is one of the earliest and pioneering work on generating likely program invariants for software programs~\cite{daikon2000ernst}. IODINE is one of the earliest work for hardware assertion generation by analyzing dynamic program behavior with respect to a set of standard property templates~\cite{iodine2005}. Prior works~\cite{pinter2005hase, wang1998dac, hekmatpour2005} have used static analysis for assertion generation whereas~\cite{rogin2008date, inferno2009tcad, chang2015aspdac, chung2011iccd} have used dynamic simulation execution data for assertion generation. $\goldmine$ introduced the novel concept of data-driven statistical analysis guided by the lightweight static analysis of design source code to automatically generate assertions for a broad spectrum of hardware designs~\cite{goldmine, hertz2013tacd}. Following $\goldmine$, researchers have developed a wide variety of assertion generation techniques
%Automated generation of hardware design properties has long been an active area of research, yielding a wide variety of techniques 
using a combination of lightweight analysis of design source code and data-driven dynamic analysis targeting design functionality~\cite{hertz2019aspdac, pal2020tcad, malburg2017aspdac, iman2024artmine, iman2021norcas, danese2017dac, germiniani2022vlsi, iman2022dsd, harm2022tcad} and design security~\cite{calvin2021ashes, hasini2023jetc}. Additionally, researchers have proposed %multiple 
approaches to evaluate the quality of numerous assertions that automatic methods generate in terms of captured design functionality and security to induce a rank order to aid the downstream verification tasks~\cite{avinash2024host, pal2020tcad, iman2022dsd, tara2015vlsisoc}. \bem{However, all these works suffer from following shortcomings} -- they (i) %they 
do not scale for industrial-scale designs, (ii) %they 
often require massive amount of %design execution 
trace data to %infer/
generate %design 
properties, (iii) %they 
generate too many design properties, often redundant, without any explanation on their usability for verification tasks, (iv) %they 
fail to generalize the properties beyond what is seen in the trace, and (v) %they 
encompass an extremely small subset of SystemVerilog (SVA) %LRM 
grammar~\cite{svmlrm}, limiting the expressibility and richness of the generated design properties. 

Recently, massive success of Large-Language Models (LLMs), \eg, GPT~\cite{openai2024gpt4}, LLaMa~\cite{touvron2023llama, llama2024web}, Gemini~\cite{gemini2024google}, in diverse applications have led researchers to investigate application of %In-Context Learning Techniques (ICL) with 
LLMs for hardware property generation %to generate functional and security properties for hardware designs
~\cite{liu2023verilogeval, orenesvera2023using, kande2023llmassisted, fang2024assertllm, mali2024chiraag, stutton2023icml}. \bem{However, almost all recent works on property generation using LLMs suffer from the following shortcomings} -- they (i) %they 
require considerable %amount of 
\fixme{human efforts and  deep %human 
understanding of the target hardware designs to devise {\em hand-crafted prompts}} to generate and refine %the functional and security 
%hardware 
hardware properties,  %necessitating a deep human understanding of the target hardware designs, 
(ii) %they 
do not generalize the assertions, and (iii) %they 
do not consider execution traces, risking to potentially miss subtle incorrect design behaviors or security vulnerabilities %issues 
that are not obvious in the design source code. In fact, there does not exist a systematic study in comparing the effectiveness of different commercial and open-source LLMs %models 
in generating valid assertions for an input Verilog hardware design. 

In this paper, we address this gap and propose $\pname$ to evaluate the goodness of four different widely-used LLMs on generating valid assertions. $\pname$ can be used to evaluate the assertion generation capabilities of any future LLMs as well. 

%Our benchmark consists %is comprised 
% of five base examples for 1-shot and 5-shot learning, where each base example is a tuple consisting of a Verilog design and its formally verified assertions, generated from $\goldmine$ and HARM, and verified using Cadence JasperGold~\cite{jaspergold}. Our test contains 100 Verilog designs OpenCores. We will detail our benchmark in~\Cref{sec:benchmark}.

%1-shot and 5-shot learning of the LLM where the base example is provided with the Verilog design and its assertions generated from GoldMine and HARM
%\assign{@Vaishnavi: details of training set including number of designs and example assertions from {\scshape GoldMine} and HARM} 
%, in the training set and 100 designs in the test set, providing a comprehensive resource for advancing in-depth research of LLMs for assertion generation task.

==> table/Results_Vaishnavi_06052024_CSV_1.tex <==
fht\_1d\_x8 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.98 & 0.02 & 0.00 & 0.91 & 0.09 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.96 & 0.04 & 0.00 & 0.89 & 0.11 & 0.00 \\
fht\_8x8\_core & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.92 & 0.08 & 0.00 & 0.89 & 0.11 & 0.00 & 0.92 & 0.08 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
fht\_bfly & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.50 & 0.50 & 0.00 & 0.67 & 0.33 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 \\
fht\_bfly\_noFF & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.25 & 0.75 & 0.00 & 0.60 & 0.40 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
mtx\_trps\_8x8\_dpsram & 0.00 & 0.00 & 1.00 & 0.75 & 0.25 & 0 & 0.93 & 0.07 & 0.00 & 0.93 & 0.07 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.80 & 0.20 & 0.00 \\
signed\_mult\_const\_asic & 0.00 & 0.00 & 1.00 & 0.75 & 0.25 & 0 & 0.63 & 0.38 & 0.00 & 0.63 & 0.38 & 0.00 & 0.00 & 1.00 & 0.00 & 0.43 & 0.57 & 0.00 & 0.40 & 0.60 & 0.00 & 0.00 & 0.00 & 1.00 \\
signed\_mult\_const\_fpga & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.20 & 0.80 & 0.00 & 0.20 & 0.80 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
accumulatorMUX & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.86 & 0.14 & 0.00 & 0.86 & 0.14 & 0.00 & 0.67 & 0.33 & 0.00 & 0.67 & 0.33 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
bitNegator & 0.67 & 0.33 & 0.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 0.00 & 1.00 \\
ramBit & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.17 & 0.83 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.20 & 0.80 & 0.00 \\ \hline
byteNegator & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
ramByte & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.25 & 0.75 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
inputReg & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.01 & 0.99 & 0.00 & 0.00 & 0.00 & 1.00 \\
outputReg & 0.33 & 0.67 & 0.00 & 1.00 & 0.00 & 0 & 0.57 & 0.43 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
ppReg1 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
tcLoad & 0.75 & 0.25 & 0.00 & 0.50 & 0.50 & 0 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.63 & 0.38 & 0.00 & 1.00 & 0.00 & 0.00 & 0.16 & 0.84 & 0.00 \\
tcReset & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0 & 0.75 & 0.25 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.14 & 0.86 & 0.00 & 0.00 & 0.00 & 1.00 \\
uartRec & 0.00 & 1.00 & 0.00 & 0.18 & 0.82 & 0 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.36 & 0.64 & 0.00 & 0.00 & 0.00 & 1.00 & 0.14 & 0.86 & 0.00 & 0.92 & 0.08 & 0.00 \\
uartTrans & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.86 & 0.14 & 0.00 & 1.00 & 0.00 & 0.00 & 0.35 & 0.65 & 0.00 & 0.00 & 0.00 & 1.00 & 0.68 & 0.32 & 0.00 & 0.53 & 0.47 & 0.00 \\
host\_interface\_aes & 0.00 & 0.00 & 1.00 & 0.21 & 0.79 & 0 & 0.64 & 0.36 & 0.00 & 0.60 & 0.40 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.31 & 0.69 & 0.00 & 0.13 & 0.88 & 0.00 \\ \hline
key\_expander & 0.38 & 0.63 & 0.00 & 0.29 & 0.71 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.28 & 0.72 & 0.00 & 0.00 & 0.00 & 1.00 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 \\
clc\_fsm & 1.00 & 0.00 & 0.00 & 0.91 & 0.09 & 0 & 0.93 & 0.07 & 0.00 & 0.93 & 0.07 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
clc\_len\_gen & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
clc\_read\_lels & 0.25 & 0.75 & 0.00 & 0.64 & 0.36 & 0 & 0.00 & 0.00 & 1.00 & 0.31 & 0.69 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.94 & 0.06 & 0.00 & 1.00 & 0.00 & 0.00 \\
clc\_read\_total\_coeffs & 0.74 & 0.26 & 0.00 & 0.36 & 0.64 & 0 & 0.64 & 0.36 & 0.00 & 0.74 & 0.26 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
clc\_read\_total\_zeros & 0.14 & 0.86 & 0.00 & 0.03 & 0.97 & 0 & 0.39 & 0.61 & 0.00 & 0.39 & 0.61 & 0.00 & 0.35 & 0.65 & 0.00 & 0.14 & 0.86 & 0.00 & 0.04 & 0.96 & 0.00 & 0.00 & 1.00 & 0.00 \\
ca\_prng & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.89 & 0.11 & 0.00 & 0.41 & 0.59 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0.00 & 0.19 & 0.81 & 0.00 \\
mux4to1 & 0.33 & 0.67 & 0.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.29 & 0.71 & 0.00 & 0.20 & 0.80 & 0.00 \\
PSGBusArb & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 0.00 & 1.00 & 0.00 & 0.11 & 0.89 & 0.00 & 0.50 & 0.50 & 0.00 & 0.94 & 0.06 & 0.00 & 0.56 & 0.44 & 0.00 & 1.00 & 0.00 & 0.00 \\
PSGChannelSummer & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\ \hline
PSGFilter & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0 & 0.09 & 0.91 & 0.00 & 0.09 & 0.91 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
PSGMasterVolumeControl & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.17 & 0.83 & 0.00 & 0.08 & 0.92 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
PSGOutputSummer & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 \\
PSGShaper & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
bit\_rersal & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.13 & 0.88 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0.00 & 0.25 & 0.75 & 0.00 \\
crc\_comb & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.94 & 0.06 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.20 & 0.80 & 0.00 \\
crc\_control\_unit & 0.59 & 0.41 & 0.00 & 0.00 & 1.00 & 0 & 1.00 & 0.00 & 0.00 & 0.93 & 0.07 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.84 & 0.16 & 0.00 & 0.93 & 0.07 & 0.00 \\
host\_interface & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0 & 0.75 & 0.25 & 0.00 & 0.79 & 0.21 & 0.00 & 0.00 & 1.00 & 0.00 & 0.63 & 0.38 & 0.00 & 0.00 & 1.00 & 0.00 & 0.64 & 0.36 & 0.00 \\
fpu\_exceptions & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.68 & 0.32 & 0.00 & 0.00 & 0.00 & 1.00 \\
fpu\_sub & 0.00 & 1.00 & 0.00 & 0.17 & 0.83 & 0 & 0.00 & 1.00 & 0.00 & 0.03 & 0.97 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\ \hline
qadd & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 0.80 & 0.20 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.75 & 0.25 & 0.00 & 0.75 & 0.25 & 0.00 & 0.00 & 0.00 & 1.00 \\
qmult & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0 & 0.89 & 0.11 & 0.00 & 0.78 & 0.22 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.95 & 0.05 & 0.00 & 0.29 & 0.71 & 0.00 \\
qtwosComp & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.10 & 0.90 & 0.00 & 0.17 & 0.83 & 0.00 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
dff\_3\_pipe & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0 & 0.50 & 0.50 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 \\
node & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 \\
dpll & 0.36 & 0.64 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.10 & 0.90 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.24 & 0.76 & 0.00 \\
freqdider & 0.00 & 1.00 & 0.00 & 0.17 & 0.83 & 0 & 0.00 & 1.00 & 0.00 & 0.20 & 0.80 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
variableresetrandomwalkfilter & 0.00 & 0.00 & 1.00 & 0.73 & 0.27 & 0 & 0.37 & 0.63 & 0.00 & 0.41 & 0.59 & 0.00 & 0.39 & 0.61 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.83 & 0.17 & 0.00 \\
clean\_rst & 0.50 & 0.50 & 0.00 & 0.67 & 0.33 & 0 & 0.33 & 0.67 & 0.00 & 0.40 & 0.60 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.60 & 0.40 & 0.00 & 0.29 & 0.71 & 0.00 \\
decoder\_8b10b & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.03 & 0.97 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.33 & 0.67 & 0.00 & 0.19 & 0.81 & 0.00 \\ \hline
encoder\_8b10b & 0.00 & 0.00 & 1.00 & 0.19 & 0.81 & 0 & 0.25 & 0.75 & 0.00 & 0.11 & 0.89 & 0.00 & 0.42 & 0.58 & 0.00 & 0.79 & 0.21 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
ge\_1000baseX\_mdio & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.71 & 0.29 & 0.00 & 0.00 & 0.00 & 1.00 \\
ge\_1000baseX\_rx & 0.19 & 0.81 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.64 & 0.36 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
ge\_1000baseX\_sync & 0.26 & 0.74 & 0.00 & 0.18 & 0.82 & 0 & 0.38 & 0.63 & 0.00 & 0.27 & 0.73 & 0.00 & 0.27 & 0.73 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.12 & 0.88 & 0.00 \\
eth\_cop & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
eth\_crc & 0.00 & 1.00 & 0.00 & 0.75 & 0.25 & 0 & 0.26 & 0.74 & 0.00 & 0.27 & 0.73 & 0.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 1.00 & 0.00 & 0.14 & 0.86 & 0.00 \\
eth\_l3\_checksum & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 \\
eth\_random & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.67 & 0.33 & 0.00 & 0.93 & 0.07 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.67 & 0.33 & 0.00 & 0.43 & 0.57 & 0.00 \\
eth\_receecontrol & 0.55 & 0.45 & 0.00 & 0.58 & 0.42 & 0 & 0.52 & 0.48 & 0.00 & 0.28 & 0.72 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.45 & 0.55 & 0.00 \\
eth\_rxaddrcheck & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 1.00 & 0.00 & 0.24 & 0.76 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\ \hline
eth\_clockgen & 0.00 & 0.00 & 1.00 & 0.67 & 0.33 & 0 & 0.60 & 0.40 & 0.00 & 0.67 & 0.33 & 0.00 & 0.00 & 1.00 & 0.00 & 0.67 & 0.33 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
eth\_miim & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.54 & 0.46 & 0.00 & 0.52 & 0.48 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
eth\_outputcontrol & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.43 & 0.57 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 & 0.14 & 0.86 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
eth\_shiftreg & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.33 & 0.67 & 0.00 & 0.20 & 0.80 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
flow\_ctrl & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0 & 0.53 & 0.47 & 0.00 & 0.10 & 0.90 & 0.00 & 0.19 & 0.81 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
MAC\_rx\_ctrl & 0.00 & 0.00 & 1.00 & 0.25 & 0.75 & 0 & 0.78 & 0.23 & 0.00 & 0.79 & 0.21 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.30 & 0.70 & 0.00 \\
Phy\_sim & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.38 & 0.63 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
Ramdon\_gen & 0.00 & 0.00 & 1.00 & 0.25 & 0.75 & 0 & 0.70 & 0.30 & 0.00 & 0.70 & 0.30 & 0.00 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 & 0.73 & 0.27 & 0.00 & 0.08 & 0.92 & 0.00 \\
reg\_int\_sim & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.71 & 0.29 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
RMON\_addr\_gen & 0.00 & 0.00 & 1.00 & 0.23 & 0.77 & 0 & 0.00 & 0.00 & 1.00 & 0.40 & 0.60 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.44 & 0.56 & 0.00 & 0.00 & 1.00 & 0.00 \\ \hline
RMON\_ctrl & 0.00 & 0.00 & 1.00 & 0.61 & 0.39 & 0 & 0.76 & 0.24 & 0.00 & 0.78 & 0.23 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.52 & 0.48 & 0.00 \\
ack\_counter & 0.00 & 0.00 & 1.00 & 0.56 & 0.44 & 0 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 & 0.17 & 0.83 & 0.00 & 0.14 & 0.86 & 0.00 & 0.10 & 0.90 & 0.00 & 0.13 & 0.87 & 0.00 \\
counter & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0 & 0.50 & 0.50 & 0.00 & 0.56 & 0.44 & 0.00 & 0.33 & 0.67 & 0.00 & 0.33 & 0.67 & 0.00 & 0.43 & 0.57 & 0.00 & 0.00 & 0.00 & 1.00 \\
rxClkgen & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 \\
rxLinkFaultState & 0.00 & 0.00 & 1.00 & 0.29 & 0.71 & 0 & 0.20 & 0.80 & 0.00 & 0.20 & 0.80 & 0.00 & 0.26 & 0.74 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0.00 \\
rxNumCounter & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0 & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.97 & 0.03 & 0.00 \\
rxStateMachine & 0.00 & 0.00 & 1.00 & 0.67 & 0.33 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.71 & 0.29 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
rxStatModule & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 0.06 & 0.94 & 0.00 & 0.06 & 0.94 & 0.00 & 0.06 & 0.94 & 0.00 & 0.06 & 0.94 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 \\
apb & 0.17 & 0.83 & 0.00 & 0.73 & 0.27 & 0 & 0.73 & 0.27 & 0.00 & 0.73 & 0.27 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.40 & 0.60 & 0.00 \\
can\_btl & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.15 & 0.85 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\ \hline
can\_crc & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.43 & 0.57 & 0.00 \\
can\_fifo & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.29 & 0.71 & 0.00 & 0.29 & 0.71 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.03 & 0.97 & 0.00 \\
can\_ibo & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
can\_register\_asyn & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
can\_register\_asyn\_syn & 0.50 & 0.50 & 0.00 & 0.25 & 0.75 & 0 & 0.40 & 0.60 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 \\
can\_register & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
can\_register\_syn & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
can\_acf & 0.00 & 1.00 & 0.00 & 0.29 & 0.71 & 0 & 0.00 & 1.00 & 0.00 & 0.14 & 0.86 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.04 & 0.96 & 0.00 \\
eth\_fifo & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.19 & 0.81 & 0.00 & 0.17 & 0.83 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
Phy\_int & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.29 & 0.71 & 0.00 & 0.31 & 0.69 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.05 & 0.95 & 0.00 \\ \hline
% fpu\_add & 0.17 & 0.83 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.08 & 0.92 & 0.00 & 0.00 & 1.00 & 0.00 & 0.15 & 0.85 & 0.00 \\
% control\_unit & 0.00 & 0.00 & 1.00 & 0.93 & 0.07 & 0 & 0.95 & 0.05 & 0.00 & 0.95 & 0.05 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 0.99 & 0.01 & 0.00 & 1.00 & 0.00 & 0.00 \\
% phasecomparator & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% wptr\_handler & 0.71 & 0.29 & 0.00 & 1.00 & 0.00 & 0 & 0.00 & 0.00 & 1.00 & 0.90 & 0.10 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.00 & 0.00 & 1.00 & 0.83 & 0.17 & 0.00 \\
% rptr\_handler & 1.00 & 0.00 & 0.00 & 0.86 & 0.14 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.89 & 0.11 & 0.00 & 0.86 & 0.14 & 0.00 \\
% synchronizer & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.60 & 0.40 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.13 & 0.88 & 0.00 & 0.11 & 0.89 & 0.00 \\
% fifo\_mem & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% MAC\_tx\_Ctrl & 0.18 & 0.82 & 0.00 & 0.00 & 1.00 & 0 & 0.67 & 0.33 & 0.00 & 0.74 & 0.26 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.58 & 0.42 & 0.00 & 0.55 & 0.45 & 0.00 \\


==> table/Results_Vaishnavi_06052024_CSV_2.tex <==
% fht\_1d\_x8 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.98 & 0.02 & 0.00 & 0.91 & 0.09 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.96 & 0.04 & 0.00 & 0.89 & 0.11 & 0.00 \\
% fht\_8x8\_core & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.92 & 0.08 & 0.00 & 0.89 & 0.11 & 0.00 & 0.92 & 0.08 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% fht\_bfly & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.50 & 0.50 & 0.00 & 0.67 & 0.33 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 \\
% fht\_bfly\_noFF & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.25 & 0.75 & 0.00 & 0.60 & 0.40 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
% mtx\_trps\_8x8\_dpsram & 0.00 & 0.00 & 1.00 & 0.75 & 0.25 & 0 & 0.93 & 0.07 & 0.00 & 0.93 & 0.07 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.80 & 0.20 & 0.00 \\
% signed\_mult\_const\_asic & 0.00 & 0.00 & 1.00 & 0.75 & 0.25 & 0 & 0.63 & 0.38 & 0.00 & 0.63 & 0.38 & 0.00 & 0.00 & 1.00 & 0.00 & 0.43 & 0.57 & 0.00 & 0.40 & 0.60 & 0.00 & 0.00 & 0.00 & 1.00 \\
% signed\_mult\_const\_fpga & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.20 & 0.80 & 0.00 & 0.20 & 0.80 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% accumulatorMUX & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.86 & 0.14 & 0.00 & 0.86 & 0.14 & 0.00 & 0.67 & 0.33 & 0.00 & 0.67 & 0.33 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% bitNegator & 0.67 & 0.33 & 0.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 0.00 & 1.00 \\
% ramBit & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.17 & 0.83 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.20 & 0.80 & 0.00 \\ \hline
% byteNegator & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% ramByte & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.25 & 0.75 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% inputReg & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.01 & 0.99 & 0.00 & 0.00 & 0.00 & 1.00 \\
% outputReg & 0.33 & 0.67 & 0.00 & 1.00 & 0.00 & 0 & 0.57 & 0.43 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% ppReg1 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% tcLoad & 0.75 & 0.25 & 0.00 & 0.50 & 0.50 & 0 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.63 & 0.38 & 0.00 & 1.00 & 0.00 & 0.00 & 0.16 & 0.84 & 0.00 \\
% tcReset & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0 & 0.75 & 0.25 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.14 & 0.86 & 0.00 & 0.00 & 0.00 & 1.00 \\
% uartRec & 0.00 & 1.00 & 0.00 & 0.18 & 0.82 & 0 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.36 & 0.64 & 0.00 & 0.00 & 0.00 & 1.00 & 0.14 & 0.86 & 0.00 & 0.92 & 0.08 & 0.00 \\
% uartTrans & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.86 & 0.14 & 0.00 & 1.00 & 0.00 & 0.00 & 0.35 & 0.65 & 0.00 & 0.00 & 0.00 & 1.00 & 0.68 & 0.32 & 0.00 & 0.53 & 0.47 & 0.00 \\
% host\_interface\_aes & 0.00 & 0.00 & 1.00 & 0.21 & 0.79 & 0 & 0.64 & 0.36 & 0.00 & 0.60 & 0.40 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.31 & 0.69 & 0.00 & 0.13 & 0.88 & 0.00 \\ \hline
% key\_expander & 0.38 & 0.63 & 0.00 & 0.29 & 0.71 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.28 & 0.72 & 0.00 & 0.00 & 0.00 & 1.00 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 \\
% clc\_fsm & 1.00 & 0.00 & 0.00 & 0.91 & 0.09 & 0 & 0.93 & 0.07 & 0.00 & 0.93 & 0.07 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
% clc\_len\_gen & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
% clc\_read\_lels & 0.25 & 0.75 & 0.00 & 0.64 & 0.36 & 0 & 0.00 & 0.00 & 1.00 & 0.31 & 0.69 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.94 & 0.06 & 0.00 & 1.00 & 0.00 & 0.00 \\
% clc\_read\_total\_coeffs & 0.74 & 0.26 & 0.00 & 0.36 & 0.64 & 0 & 0.64 & 0.36 & 0.00 & 0.74 & 0.26 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
% clc\_read\_total\_zeros & 0.14 & 0.86 & 0.00 & 0.03 & 0.97 & 0 & 0.39 & 0.61 & 0.00 & 0.39 & 0.61 & 0.00 & 0.35 & 0.65 & 0.00 & 0.14 & 0.86 & 0.00 & 0.04 & 0.96 & 0.00 & 0.00 & 1.00 & 0.00 \\
% ca\_prng & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.89 & 0.11 & 0.00 & 0.41 & 0.59 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0.00 & 0.19 & 0.81 & 0.00 \\
% mux4to1 & 0.33 & 0.67 & 0.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.29 & 0.71 & 0.00 & 0.20 & 0.80 & 0.00 \\
% PSGBusArb & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 0.00 & 1.00 & 0.00 & 0.11 & 0.89 & 0.00 & 0.50 & 0.50 & 0.00 & 0.94 & 0.06 & 0.00 & 0.56 & 0.44 & 0.00 & 1.00 & 0.00 & 0.00 \\
% PSGChannelSummer & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\ \hline
% PSGFilter & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0 & 0.09 & 0.91 & 0.00 & 0.09 & 0.91 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% PSGMasterVolumeControl & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.17 & 0.83 & 0.00 & 0.08 & 0.92 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% PSGOutputSummer & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 \\
% PSGShaper & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% bit\_rersal & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.13 & 0.88 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0.00 & 0.25 & 0.75 & 0.00 \\
% crc\_comb & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.94 & 0.06 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.20 & 0.80 & 0.00 \\
% crc\_control\_unit & 0.59 & 0.41 & 0.00 & 0.00 & 1.00 & 0 & 1.00 & 0.00 & 0.00 & 0.93 & 0.07 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.84 & 0.16 & 0.00 & 0.93 & 0.07 & 0.00 \\
% host\_interface & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0 & 0.75 & 0.25 & 0.00 & 0.79 & 0.21 & 0.00 & 0.00 & 1.00 & 0.00 & 0.63 & 0.38 & 0.00 & 0.00 & 1.00 & 0.00 & 0.64 & 0.36 & 0.00 \\
% fpu\_exceptions & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.68 & 0.32 & 0.00 & 0.00 & 0.00 & 1.00 \\
% fpu\_sub & 0.00 & 1.00 & 0.00 & 0.17 & 0.83 & 0 & 0.00 & 1.00 & 0.00 & 0.03 & 0.97 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\ \hline
% qadd & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 0.80 & 0.20 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.75 & 0.25 & 0.00 & 0.75 & 0.25 & 0.00 & 0.00 & 0.00 & 1.00 \\
% qmult & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0 & 0.89 & 0.11 & 0.00 & 0.78 & 0.22 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.95 & 0.05 & 0.00 & 0.29 & 0.71 & 0.00 \\
% qtwosComp & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.10 & 0.90 & 0.00 & 0.17 & 0.83 & 0.00 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% dff\_3\_pipe & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0 & 0.50 & 0.50 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 \\
% node & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 \\
% dpll & 0.36 & 0.64 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.10 & 0.90 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.24 & 0.76 & 0.00 \\
% freqdider & 0.00 & 1.00 & 0.00 & 0.17 & 0.83 & 0 & 0.00 & 1.00 & 0.00 & 0.20 & 0.80 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% variableresetrandomwalkfilter & 0.00 & 0.00 & 1.00 & 0.73 & 0.27 & 0 & 0.37 & 0.63 & 0.00 & 0.41 & 0.59 & 0.00 & 0.39 & 0.61 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.83 & 0.17 & 0.00 \\
% clean\_rst & 0.50 & 0.50 & 0.00 & 0.67 & 0.33 & 0 & 0.33 & 0.67 & 0.00 & 0.40 & 0.60 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.60 & 0.40 & 0.00 & 0.29 & 0.71 & 0.00 \\
% decoder\_8b10b & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.03 & 0.97 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.33 & 0.67 & 0.00 & 0.19 & 0.81 & 0.00 \\ \hline
% encoder\_8b10b & 0.00 & 0.00 & 1.00 & 0.19 & 0.81 & 0 & 0.25 & 0.75 & 0.00 & 0.11 & 0.89 & 0.00 & 0.42 & 0.58 & 0.00 & 0.79 & 0.21 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% ge\_1000baseX\_mdio & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.71 & 0.29 & 0.00 & 0.00 & 0.00 & 1.00 \\
% ge\_1000baseX\_rx & 0.19 & 0.81 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.64 & 0.36 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
% ge\_1000baseX\_sync & 0.26 & 0.74 & 0.00 & 0.18 & 0.82 & 0 & 0.38 & 0.63 & 0.00 & 0.27 & 0.73 & 0.00 & 0.27 & 0.73 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.12 & 0.88 & 0.00 \\
% eth\_cop & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% eth\_crc & 0.00 & 1.00 & 0.00 & 0.75 & 0.25 & 0 & 0.26 & 0.74 & 0.00 & 0.27 & 0.73 & 0.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 1.00 & 0.00 & 0.14 & 0.86 & 0.00 \\
% eth\_l3\_checksum & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 \\
% eth\_random & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.67 & 0.33 & 0.00 & 0.93 & 0.07 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.67 & 0.33 & 0.00 & 0.43 & 0.57 & 0.00 \\
% eth\_receecontrol & 0.55 & 0.45 & 0.00 & 0.58 & 0.42 & 0 & 0.52 & 0.48 & 0.00 & 0.28 & 0.72 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.45 & 0.55 & 0.00 \\
% eth\_rxaddrcheck & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 1.00 & 0.00 & 0.24 & 0.76 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\ \hline
% eth\_clockgen & 0.00 & 0.00 & 1.00 & 0.67 & 0.33 & 0 & 0.60 & 0.40 & 0.00 & 0.67 & 0.33 & 0.00 & 0.00 & 1.00 & 0.00 & 0.67 & 0.33 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% eth\_miim & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.54 & 0.46 & 0.00 & 0.52 & 0.48 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% eth\_outputcontrol & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.43 & 0.57 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 & 0.14 & 0.86 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% eth\_shiftreg & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.33 & 0.67 & 0.00 & 0.20 & 0.80 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% flow\_ctrl & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0 & 0.53 & 0.47 & 0.00 & 0.10 & 0.90 & 0.00 & 0.19 & 0.81 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% MAC\_rx\_ctrl & 0.00 & 0.00 & 1.00 & 0.25 & 0.75 & 0 & 0.78 & 0.23 & 0.00 & 0.79 & 0.21 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.30 & 0.70 & 0.00 \\
% Phy\_sim & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.38 & 0.63 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
% Ramdon\_gen & 0.00 & 0.00 & 1.00 & 0.25 & 0.75 & 0 & 0.70 & 0.30 & 0.00 & 0.70 & 0.30 & 0.00 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 & 0.73 & 0.27 & 0.00 & 0.08 & 0.92 & 0.00 \\
% reg\_int\_sim & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.71 & 0.29 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
% RMON\_addr\_gen & 0.00 & 0.00 & 1.00 & 0.23 & 0.77 & 0 & 0.00 & 0.00 & 1.00 & 0.40 & 0.60 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.44 & 0.56 & 0.00 & 0.00 & 1.00 & 0.00 \\ \hline
% RMON\_ctrl & 0.00 & 0.00 & 1.00 & 0.61 & 0.39 & 0 & 0.76 & 0.24 & 0.00 & 0.78 & 0.23 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.52 & 0.48 & 0.00 \\
% ack\_counter & 0.00 & 0.00 & 1.00 & 0.56 & 0.44 & 0 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 & 0.17 & 0.83 & 0.00 & 0.14 & 0.86 & 0.00 & 0.10 & 0.90 & 0.00 & 0.13 & 0.87 & 0.00 \\
% counter & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0 & 0.50 & 0.50 & 0.00 & 0.56 & 0.44 & 0.00 & 0.33 & 0.67 & 0.00 & 0.33 & 0.67 & 0.00 & 0.43 & 0.57 & 0.00 & 0.00 & 0.00 & 1.00 \\
% rxClkgen & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 \\
% rxLinkFaultState & 0.00 & 0.00 & 1.00 & 0.29 & 0.71 & 0 & 0.20 & 0.80 & 0.00 & 0.20 & 0.80 & 0.00 & 0.26 & 0.74 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0.00 \\
% rxNumCounter & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0 & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.97 & 0.03 & 0.00 \\
% rxStateMachine & 0.00 & 0.00 & 1.00 & 0.67 & 0.33 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.71 & 0.29 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% rxStatModule & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 0.06 & 0.94 & 0.00 & 0.06 & 0.94 & 0.00 & 0.06 & 0.94 & 0.00 & 0.06 & 0.94 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 \\
% apb & 0.17 & 0.83 & 0.00 & 0.73 & 0.27 & 0 & 0.73 & 0.27 & 0.00 & 0.73 & 0.27 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.40 & 0.60 & 0.00 \\
% can\_btl & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.15 & 0.85 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\ \hline
% can\_crc & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.43 & 0.57 & 0.00 \\
% can\_fifo & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.29 & 0.71 & 0.00 & 0.29 & 0.71 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.03 & 0.97 & 0.00 \\
% can\_ibo & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
% can\_register\_asyn & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% can\_register\_asyn\_syn & 0.50 & 0.50 & 0.00 & 0.25 & 0.75 & 0 & 0.40 & 0.60 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 \\
% can\_register & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% can\_register\_syn & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% can\_acf & 0.00 & 1.00 & 0.00 & 0.29 & 0.71 & 0 & 0.00 & 1.00 & 0.00 & 0.14 & 0.86 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.04 & 0.96 & 0.00 \\
% eth\_fifo & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.19 & 0.81 & 0.00 & 0.17 & 0.83 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% Phy\_int & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.29 & 0.71 & 0.00 & 0.31 & 0.69 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.05 & 0.95 & 0.00 \\ \hline
fpu\_add & 0.17 & 0.83 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.08 & 0.92 & 0.00 & 0.00 & 1.00 & 0.00 & 0.15 & 0.85 & 0.00 \\
control\_unit & 0.00 & 0.00 & 1.00 & 0.93 & 0.07 & 0 & 0.95 & 0.05 & 0.00 & 0.95 & 0.05 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 0.99 & 0.01 & 0.00 & 1.00 & 0.00 & 0.00 \\
phasecomparator & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
wptr\_handler & 0.71 & 0.29 & 0.00 & 1.00 & 0.00 & 0 & 0.00 & 0.00 & 1.00 & 0.90 & 0.10 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.00 & 0.00 & 1.00 & 0.83 & 0.17 & 0.00 \\
rptr\_handler & 1.00 & 0.00 & 0.00 & 0.86 & 0.14 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.89 & 0.11 & 0.00 & 0.86 & 0.14 & 0.00 \\
synchronizer & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.60 & 0.40 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.13 & 0.88 & 0.00 & 0.11 & 0.89 & 0.00 \\
fifo\_mem & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
MAC\_tx\_Ctrl & 0.18 & 0.82 & 0.00 & 0.00 & 1.00 & 0 & 0.67 & 0.33 & 0.00 & 0.74 & 0.26 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.58 & 0.42 & 0.00 & 0.55 & 0.45 & 0.00 \\ \hline


==> table/design_summary.tex <==
\begin{table*}
    \centering
    \caption{{\bf Details of a few representative designs in the test set of $\pname$ benchmark}.}
    \label{tab:design_details}    
    \begin{tabular}{l|ll|p{5.2cm}}
        \hline
        {\bf Verilog Design} & {\bf \# of Lines} &  {\bf Design Type} & {\bf Design Functionality} \\ 
        \hline\hline
        ca\_prng & 1144 &  Sequential &  A compact Pattern Generator  \\%capable of providing user selectable patterns at GByte/s speed. \\ 
        \hline
        cavlc\_read\_total\_coeffs & 1090 & Sequential & %This is one of the designs used for 
        Video Encoder %coding 
        for generic audio visual. \\
        \hline
        cavlc\_read\_total\_zeros & 637 & Combinational & Video Encoder for generic audio visual. \\
        %This is one of the designs used for video coding for generic audiovisual \\
        \hline
        ge\_1000baseX\_rx &	544 & Sequential & Verilog implementation of Physical Coding Sublayer (PCS) type. \\
        \hline
        MAC\_tx\_Ctrl & 504 & Sequential &   An Ethernet MAC controller. \\ %conforming to IEEE 802.3 specification \\
        \hline
    \end{tabular}
\end{table*}

==> table/post_syntactic_correction.tex <==
\begin{table}
    \centering
    \caption{{\bf Comparative results for four different commercial and open-source LLMs using 1-shot and 5-shot learning for the assertion generation task}. {\bf P}: Fraction of proven assertions. {\bf C}: Fraction of failed assertions with a counter example. {\bf E}: Fraction of assertions which have syntax errors.}
    \label{tab:result_after_syn_correction}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
         \hline
         \multirow{2}{*}{\bf Designs} & \multicolumn{6}{|c|}{\bf ChatGPT 3.5} & \multicolumn{6}{|c|}{\bf ChatGPT 4.0} & \multicolumn{6}{|c|}{\bf CodeLLaMa2} & \multicolumn{6}{|c|}{\bf LLaMa3-70B} \\
         \cline{2-25}
         \multirow{2}{*}{} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} \\
         \cline{2-25}
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E}
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E} \\
         \hline
         \input{table/Results_Vaishnavi_06052024_CSV_1}
    \end{tabular}
    }
\end{table}

\begin{table}
    \centering
    \caption{{\bf Comparative results for four different commercial and open-source LLMs using 1-shot and 5-shot learning for the assertion generation task}. {\bf P}: Fraction of proven assertions. {\bf C}: Fraction of failed assertions with a counter example. {\bf E}: Fraction of assertions which have syntax errors.}
    \label{tab:result_after_syn_correction}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
         \hline
         \multirow{2}{*}{\bf Designs} & \multicolumn{6}{|c|}{\bf ChatGPT 3.5} & \multicolumn{6}{|c|}{\bf ChatGPT 4.0} & \multicolumn{6}{|c|}{\bf CodeLLaMa2} & \multicolumn{6}{|c|}{\bf LLaMa3-70B} \\
         \cline{2-25}
         \multirow{2}{*}{} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} \\
         \cline{2-25}
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E}
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E} \\
         \hline
         \input{table/Results_Vaishnavi_06052024_CSV_2}
         %\hline
    \end{tabular}
    }
\end{table}
